Magnetohydrodynamic structure of a plasmoid in fast reconnection in low-beta plasmas: Shock-shock interactions

The shock structure of a plasmoid in magnetic reconnection in low-beta plasmas is investigated by two-dimensional magnetohydrodynamic simulations. Using a high-accuracy code with unprecedented resolution, shocks, discontinuities, and their intersections are resolved and clarified. Contact discontinuities emanate from triple-shock intersection points, separating fluids of different origins. Shock-diamonds inside the plasmoid appear to decelerate a supersonic flow. New shock-diamonds and a slow expansion fan are found inside the Petschek outflow. A sufficient condition for the new shock-diamonds and the relevance to astrophysical jets are discussed.

==> ancillary_files/Makefile <==
F90 = gfortran -O2 -m64 -Wall
F90 = ftn
F90 = /opt/openmpi64i/bin/mpif90

OBJS = model.o set_dt.o set_dt2.o set_eta.o u2v.o input.o output.o \
	rk21.o rk22.o step1.o step2.o bc.o \
	v2u.o v2f.o v2g.o limiter_f.o limiter_g.o bc_fixv_g.o \
	hll_resistive_f.o hll_resistive_g.o \
	hlld_resistive_f.o hlld_resistive_g.o \
	glm_f.o glm_g.o glm_ss.o
OBJP = modelp.o  mpibc.o  mpi_fixv_f.o
OBJP2= modelp2.o mpibc2.o mpi_fixv_f2.o bc_fixv_g2.o

all: run runp runp2

# serial version
run : main.o $(OBJS)
	$(F90) -o a.out main.o $(OBJS)

# parallel version
runp : mainp.o $(OBJS) $(OBJP)
	$(F90) -o ap.out mainp.o $(OBJS) $(OBJP)

# parallel version (1/4 BC for large-scale evolution)
runp2 : mainp2.o $(OBJS) $(OBJP2)
	$(F90) -o ap2.out mainp2.o $(OBJS) $(OBJP2)

%.o: %.f90 param.h
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f *.out *.o data/*.dat data/*.dat.restart

